RRWaveNet: A Compact End-to-End Multi-Scale Residual CNN for Robust PPG Respiratory Rate Estimation

Respiratory rate (RR) is an important biomarker as RR changes can reflect severe medical events such as heart disease, lung disease, and sleep disorders. Unfortunately, standard manual RR counting is prone to human error and cannot be performed continuously. This study proposes a method for continuously estimating RR, RRWaveNet. The method is a compact end-to-end deep learning model which does not require feature engineering and can use low-cost raw photoplethysmography (PPG) as input signal. RRWaveNet was tested subject-independently and compared to baseline in four datasets (BIDMC, CapnoBase, WESAD, and SensAI) and using three window sizes (16, 32, and 64 seconds). RRWaveNet outperformed current state-of-the-art methods with mean absolute errors at optimal window size of 1.66 \pm 1.01, 1.59 \pm 1.08, 1.92 \pm 0.96 and 1.23 \pm 0.61 breaths per minute for each dataset. In remote monitoring settings, such as in the WESAD and SensAI datasets, we apply transfer learning to improve the performance using two other ICU datasets as pretraining datasets, reducing the MAE by up to 21$\%$. This shows that this model allows accurate and practical estimation of RR on affordable and wearable devices. Our study also shows feasibility of remote RR monitoring in the context of telemedicine and at home.

==> content/authorlist.tex <==

\author{Payongkit Lakhan, Nannapas Banluesombatkul, Natchaya Sricom, Korn Surapat, Ratha Rotruchiphong, Phattarapong Sawangjai, Tohru Yagi, Tulaya Limpiti$^{*}$ and Theerawit Wilaiprasitporn$^{*}$, \IEEEmembership{Member, IEEE}


\thanks{This work was supported by PTT Public Company Limited, The SCB Public Company Limited, The Office of the Permanent Secretary of the Ministry of Higher Education, Science, Research and Innovation, Thailand (RGNS63-252) and National Research Council of Thailand (N41A640131)  \textit{($^{*}$co-corresponding authors: Theerawit Wilaiprasitporn and Tulaya Limpiti).}}
\thanks{P. Lakhan, N. Banluesombatkul, N. Sricom and T. Wilaiprasitporn are with Bio-inspired Robotics and Neural Engineering (BRAIN) Lab, School of Information Science and Technology (IST), Vidyasirimedhi Institute of Science \& Technology (VISTEC), Rayong, Thailand (e-mail: theerawit.w@vistec.ac.th).}
\thanks{T. Limpiti are with the School of Engineering, King Mongkut's Institute of Technology Ladkrabang, Thailand. (e-mail:tulaya.li@kmitl.ac.th)}
\thanks{K. Surapat and R. Rotruchiphong are with Kamnoetvidya Science Academy School, Rayong, Thailand.}
\thanks{T. Yagi are with Yagi Lab, Department of Mechanical Engineering, Tokyo Institute of Technology, Tokyo, Japan.}
}

